Structured Chain-of-Thought Prompting for Code Generation

Large Language Models (LLMs) (e.g., ChatGPT) have shown impressive performance in code generation. LLMs take prompts as inputs, and Chain-of-Thought (CoT) prompting is the state-of-the-art prompting technique. CoT prompting asks LLMs first to generate CoTs (i.e., intermediate natural language reasoning steps) and then output the code. However, CoT prompting is designed for natural language generation and has low accuracy in code generation. In this paper, we propose Structured CoTs (SCoTs) and present a novel prompting technique for code generation, named SCoT prompting. Our motivation is source code contains rich structural information and any code can be composed of three program structures (i.e., sequence, branch, and loop structures). Intuitively, structured intermediate reasoning steps make for structured source code. Thus, we ask LLMs to use program structures to build CoTs, obtaining SCoTs. Then, LLMs generate the final code based on SCoTs. Compared to CoT prompting, SCoT prompting explicitly constrains LLMs to think about how to solve requirements from the view of source code and further the performance of LLMs in code generation. We apply SCoT prompting to two LLMs (i.e., ChatGPT and Codex) and evaluate it on three benchmarks (i.e., HumanEval, MBPP, and MBCPP). (1) SCoT prompting outperforms the state-of-the-art baseline - CoT prompting by up to 13.79% in Pass@1. (2) Human evaluation shows human developers prefer programs from SCoT prompting. (3) SCoT prompting is robust to examples and achieves substantial improvements.

==> chapter/2-Background.tex <==
\section{Background}
\label{sec:background}

\textbf{Prompting Techniques.}
Large Language Models (LLMs) for source code have been expanded and shown state-of-the-art results on code generation. Different from previous approaches, LLMs often are very large-scale (\ie Codex contains 175 billion parameters). Thus, we can not directly fine-tune LLMs on code generation.
Prompting techniques are emerging approaches to transferring LLMs into code generation. Prompting techniques do not require updating LLMs' parameters and directly enter a prompt into LLMs. Early, a prompt consists of $k$ requirement-code examples and a new requirement. By learning from examples, LLMs analogously generate a new program. When $k=0$, it is named \textit{zero-shot prompting}, and when $k>0$, it is called \textit{few-shot prompting}.



==> chapter/2-motivating_example.tex <==
\section{Motivating Example}
\label{sec:motivating_ex}

\begin{figure}[t]
\centering
\includegraphics[width=0.85\linewidth]{figure/motivating_example.pdf}
\caption{Motivating Examples of our \method.}
\label{fig:motivating_example}
\vspace{-0.4cm}
\end{figure}

In Figure \ref{fig:motivating_example}, we show some programs generated by previous approaches and our \method. In this section, we explain our motivations through these cases.

\textbf{(1) Directly generating programs from requirements is hard.} 
Previous studies leverage LLMs to directly generate programs from requirements and are prone to generate incorrect programs. For example, a representative LLM - CodeGen-16B \cite{CodeGen} only achieves 26.43\% Pass@1 in HumanEval \cite{Codex}. Even the SOTA LLM - ChatGPT \cite{ChatGPT} only obtains 52.47\% Pass@1.
Figure \ref{fig:motivating_example} shows an incorrect program generated by ChatGPT. We can see that ChatGPT mistakenly understands requirements and generates an erroneous condition statement that is highlighted. 
Thus, how to improve the performance of LLMs in code generation is still an open question.

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figure/overview.pdf}
\caption{An overview of our \method. Given a requirement, it focus on thinking about a solving process with programming logic, generating a code sketch. Then, it implements the sketch into a program using specific programming languages.}
\label{fig:overview}
\end{figure*}

\textbf{(2) Programming thinking is beneficial for LLMs to generate correct programs.}
A large-scale study found that writing a program requires the \textit{programming thinking}, \ie analyzing and implementing requirements in programming logic (\eg branch, loop).
Inspired by this finding, we propose a novel approach named \method to unlock the programming thinking of LLMs in code generation. \method decomposes code generation into two steps and progressively leads LLMs to analyze\&implement requirements in programming logic.

Given a requirement, \method first think about a rough solving process in programming logic and leaves implementation details to the future. Figure \ref{fig:motivating_example} shows a code sketch example. The sketch leverages some control statements to build a well-formed solving algorithm. Besides, it uses natural languages to accurately describe specific details, such as the span highlighted in green.

Next, \method thinks about how to implement the program and converts the sketch into a program. \method will understand the sketch and implement each step in the sketch into a code snippet. Figure \ref{fig:motivating_example} shows a correct program generated by \method. \method utilizes a library - \texttt{re} to implement the highlighted content in the sketch. It allows the \method to focus on implementing a program in a standardized way, improving the syntactic correctness of final programs.


% Given a requirement, developers first think about how to solve the requirement. For example, they will design the input-output form, overall steps of desired programs, and so on. These designed results are further organized into a syntax-free algorithm to guide the following coding process.
% Figure \ref{fig:motivating_example} shows an algorithm example. Developers use keywords (\eg \texttt{for \_ do:}) to build the algorithm structure and utilize natural language descriptions (span \#1 and \#2 in Figure \ref{fig:motivating_example}) to describe details.
% It allows developers to focus on thinking about the solving process and leave implementation details to the future.
% Next, developers focus on coding and convert the algorithm into an executable program using a programming language (\eg Python).
% As shown in Figure \ref{fig:motivating_example}, developers leverage specific APIs and libraries to implement the algorithm. The span \#1 is converted into \texttt{text.split()}, and the span \#2 is implemented by a third-party library \texttt{re}.
% By considering the algorithm as an intermediate point, developers ensure the correctness of programs in terms of logic and implementation in different stages.

% Inspired by the above process, we propose a design-and-coding approach for code generation named \method. \method first acts as a designer to design a high-level algorithm, and then acts as a coder to generate a program based on the algorithm. Experimental results show the effectiveness of our design-and-coding approach.

% \ding{183} \textbf{A algorithm is beneficial for developers to understand the functionality of programs.}
% In practice, developers use code generation tools to generate programs and spend time reviewing generated programs. As shown in Figure \ref{fig:motivating_example}, the generated code contains a complex regular expression, which will cost developers lots of effort to read and maintain the code. 

% To deal with this problem, our approach first outputs the easy-to-understand algorithm as an intermediate result and then generates a complete program. The algorithm clearly explains what each part of the code does. In practice, developers can quickly understand programs from our approach through the generated algorithm. Thus, our approach is user-friendly and the generated programs have good readability.

